WildBench: Benchmarking LLMs with Challenging Tasks from Real Users in the Wild

We introduce WildBench, an automated evaluation framework designed to benchmark large language models (LLMs) using challenging, real-world user queries. WildBench consists of 1,024 tasks carefully selected from over one million human-chatbot conversation logs. For automated evaluation with WildBench, we have developed two metrics, WB-Reward and WB-Score, which are computable using advanced LLMs such as GPT-4-turbo. WildBench evaluation uses task-specific checklists to evaluate model outputs systematically and provides structured explanations that justify the scores and comparisons, resulting in more reliable and interpretable automatic judgments. WB-Reward employs fine-grained pairwise comparisons between model responses, generating five potential outcomes: much better, slightly better, slightly worse, much worse, or a tie. Unlike previous evaluations that employed a single baseline model, we selected three baseline models at varying performance levels to ensure a comprehensive pairwise evaluation. Additionally, we propose a simple method to mitigate length bias, by converting outcomes of ``slightly better/worse'' to ``tie'' if the winner response exceeds the loser one by more than $K$ characters. WB-Score evaluates the quality of model outputs individually, making it a fast and cost-efficient evaluation metric. WildBench results demonstrate a strong correlation with the human-voted Elo ratings from Chatbot Arena on hard tasks. Specifically, WB-Reward achieves a Pearson correlation of 0.98 with top-ranking models. Additionally, WB-Score reaches 0.95, surpassing both ArenaHard's 0.91 and AlpacaEval2.0's 0.89 for length-controlled win rates, as well as the 0.87 for regular win rates.

==> correlation.tex <==

\begin{table}[t]
     \centering
     % \vspace{-2em}
    \caption{\label{tab:cor}Correlation with Chatbot ArenaElo Elo (Hard-En-240520) of alignment benchmarks.}  
    % \hspace{-2.3em}
    \scalebox{0.85}{
        \begin{tabular}{@{}ccccc||cccc@{}}
            \toprule
            Metric                        & P-Cor$_{\text{top}}$ & P-Cor$_{\text{all}}$ & S-Cor$_{\text{all}}$ & K-Cor$_{\text{all}}$ & Metric     & P-Cor$_{\text{top}}$ & P-Cor$_{\text{all}}$ &  S-Cor$_{\text{all}}$ \\
            \midrule  
            \rowcolor{lightgray}\hspace{0.3cm} ArenaElo {\small (Hard-En)} & 1.000 & 1.000 & 1.000 & 1.000 & Avg Length & 0.472 & 0.554 & 0.376 \\  \midrule
            Arena-Hard & \textit{0.909} & 0.925 & \textit{0.965} & \textit{0.890} & WB-{\small{Reward}}$^{\text{llama}}_{\infty}$ & 0.976 & 0.965 & 0.965 \\  
            AlpacaEval2-LC & 0.892 & 0.951 & 0.924 & 0.818 & WB-{\small{Reward}}$^{\text{gpt4t}}_{\infty}$ & 0.974 & 0.961 & 0.965 \\ 
            AlpacaEval2 & 0.865 & \textit{0.952} & 0.960 & 0.868 & WB-{\small{Reward}}$^{\text{haiku}}_{\infty}$ & \textbf{0.985} & \textbf{0.974} & \textbf{0.982 }\\  \midrule
            WB-{\small{Score}} & 0.955 & 0.940 & 0.943 & 0.846 & WB-{\small{Reward}}$^{\text{llama}}_{500}$ & 0.977 & 0.969 & 0.961 \\ 
            WB-{\small{Reward}}$^{\text{mix}}_{\infty}$ & \textbf{0.984} & 0.973 & \textbf{0.978} & \textbf{0.912} & WB-{\small{Reward}}$^{\text{gpt4t}}_{500}$ & \textbf{0.992} & 0.973 & 0.969 \\ 
            WB-{\small{Reward}}$^{\text{mix}}_{500}$ & \textbf{0.984 }& \textbf{0.976} & 0.974 & \textbf{0.912} & WB-{\small{Reward}}$^{\text{haiku}}_{500}$ & 0.973 & \textbf{0.976} & \textbf{0.974} \\
            \bottomrule            
        \end{tabular}
    }
\end{table}

==> leaderboard.tex <==

\begin{table}[t]
    \vspace{-2em}   
     \centering
    \caption{\label{tab:main}
    % \hspace{-2.2em}
    Evaluation results (subset) of LLMs using \wildbench{} and other benchmarks.
    Please refer to Figure~\ref{fig:leaderboard}-\ref{fig:leaderboard_new} and demo website to view and interact with the full results. 
    % \yuchen{Update link to make it anoyomous..}
    }
    % \hspace{-1.5em}
    \scalebox{0.88}{ 
        \begin{tabular}{@{}r|@{ }r@{ }|c@{ }c@{ }c@{ }c@{ }|@{ }c@{ }||c|c|c@{ }c@{}}
        \toprule
        &
        \multicolumn{1}{c|}{\multirow{2}[2]{*}{\textbf{Model names}}} & 
        \multicolumn{4}{c}{\textbf{WB-Reward} {{\small{(no length penalty)}}}} & 
        \multicolumn{1}{c||}{\textbf{WB-}} & 
        \multicolumn{1}{c|}{\textbf{Arena}} & 
        \multicolumn{1}{c|}{\textbf{Arena-}} & 
        \multicolumn{2}{c}{\textbf{AlpacaEval2}} \\  
      &  & \textbf{Mix} & \textbf{{\tiny \faBullseye}GPT4T} & \textbf{{\tiny \faBullseye}Haiku} & \textbf{{\tiny \faBullseye}Llama2} & \textbf{Score} & \textbf{Elo} & \textbf{Hard} & LC & WR \\ 
        \midrule 
  1 & GPT-4o-0513 \faLock         &             35.7 &        1.5 &       46.3 &        59.3 &       65.3 & 1293       & -           & 57.5       & 51.3     \\
 2 & {\tiny \faBullseye} GPT-4-Turbo-0409 \faLock    &             34.6 &        \textit{\textbf{0}}   &       45.3 &        58.4 &       64.7 & 1251       & 82.6        & 55.0       & 46.1     \\
 3 & GPT-4-Turbo-0125 \faLock        &             29.9 &       -4.4 &       38.8 &        55.2 &       63.3 & 1239       & 78.0        & -          & -        \\
 4 & Gemini-1.5-Pro \faLock            &             27.8 &       -4.4 &       37.9 &        50   &       55.7 & -          & -           & -          & -        \\
 5 & Llama-3-70B-Inst      &             21   &      -19   &       31.9 &        50.2 &       60.4 & 1213       & 41.1        & 34.4       & 33.2     \\
 6 & Claude 3 Opus \faLock             &             20.1 &      -20.4 &       34.3 &        46.3 &       63.1 & 1232       & 60.4        & 40.5       & 29.1     \\
 7 & Gemini-1.5-Flash \faLock           &             17.4 &      -16.6 &       26.3 &        42.5 &       53.1 & -          & -           & -          & -        \\
 8 & Yi-1.5-34B-Chat           &             16.8 &      -18.3 &       24.1 &        44.5 &       57.8 & -          & -           & -          & -        \\
 10 & Llama3-Inst-8B-SimPO &             14   &      -22.5 &       18.9 &        45.7 &       53.9 & -          & 33.8        & 44.7       & 40.5     \\
 13 & Claude 3 Sonnet \faLock           &              7.2 &      -31.6 &       19.4 &        33.9 &       55.5 & 1187       & 46.8        & 34.9       & 25.6     \\
 14 & Qwen1.5-72B-Chat          &              4.4 &      -34.8 &       13.1 &        34.7 &       56.5 & 1143       & 36.1        & 36.6       & 26.5     \\
 % 1 &  Qwen2-72B-Inst        &              3.1 &      -35.7 &       11.7 &        33.4 &       56.8 & -          & -           & -          & -        \\
% 1 &   Yi-1.5-9B-Chat            &              2   &      -32.1 &        8.7 &        29.5 &       51.8 & -          & -           & -          & -        \\
 17 & Command-R-Plus \faLock            &              0.4 &      -36.3 &        7.4 &        30.2 &       51.4 & 1155       & 33.1        & -          & -        \\ \midrule 
% 1 &   SELM (Zephyr-7B-iter3)    &             -6.8 &      -39.6 &       -3.1 &        22.2 &       46.9 & -          & -           & 24.0       & -        \\ 
20 & {\tiny \faBullseye} Claude 3 Haiku \faLock            &             -8.5 &      -46.9 &        \textit{\textbf{0}}   &        21.4 &       50.4 & 1169       & 41.5        & -          & -        \\ 
 21 & Mistral-Large \faLock             &            -10.5 &      -48.1 &       -4   &        20.5 &       54.2 & 1158       & 37.7        & 32.7       & 21.4     \\
 23 & StarlingLM-7B-beta        &            -11.9 &      -48.7 &       -5   &        18   &       46.8 & 1111       & 23.0        & -          & -        \\
 24 & Llama-3-8B-Inst       &            -14.6 &      -49.8 &       -9.7 &        15.7 &       45.7 & 1144       & 20.6        & 22.9       & 22.6     \\
 25 & Command-R \faLock                 &            -16   &      -48.4 &      -12.7 &        13.1 &       45.7 & 1106       & 17.0        & -          & -        \\
 26 & Mixtral-8x7B-Inst     &            -18.8 &      -53.4 &      -13.5 &        10.4 &       47.8 & 1114       & 23.4        & 23.7       & 18.3     \\
 27 & DBRX Inst             &            -21.6 &      -57.3 &      -16.3 &         8.7 &       48.9 & 1106       & 23.9        & 25.4       & 18.4     \\
 29 & Yi-1.5-6B-Chat            &            -24.3 &      -55   &      -19.9 &         2.1 &       39.6 & -          & -           & -          & -        \\
 30 & Mistral-7B-Inst-v0.2  &            -25   &      -58.1 &      -22.4 &         5.5 &       43.4 & 1071       & -           & 17.1       & 14.7     \\
 32 & Tulu-2-dpo-70b            &            -25.4 &      -59.3 &      -20.3 &         3.3 &       45.2 & 1099       & 15.0        & 21.2       & 16.0     \\ \midrule
 33 & {\tiny \faBullseye} Llama-2-70B-chat          &            -26.8 &      -56.9 &      -23.6 &         \textit{\textbf{0}}   &       39.2 & 1070       & 11.6        & 14.7       & 13.9     \\ 
 34 & Qwen1.5-7B-Chat           &            -27   &      -57.7 &      -23   &        -0.2 &       40   & 1059       & -           & 14.7       & 11.8     \\
 35 & Phi-3-medium-128k         &            -33.3 &      -66.4 &      -30   &        -3.6 &       42.1 & -          & -           & -          & -        \\
 36 & GPT-3.5-turbo-0125        &            -33.5 &      -66.3 &      -30   &        -4.1 &       42.1 & 1105       & 23.3        & -          & -        \\
%  37 & Phi-3-mini-128k           &            -38.3 &      -68.3 &      -35.5 &       -10.9 &       38.2 & -          & 15.4        & -          & -        \\
 38 & Llama-2-7B-chat           &            -48   &      -71.8 &      -44.6 &       -27.8 &       27.6 & 1012       & 4.6         & 5.4        & 5.0      \\
 39 & Gemma-7B-it               &            -57   &      -78.4 &      -55.8 &       -36.8 &       23.9 & 1047       & 7.5         & 10.4       & 6.9      \\
 40 & Gemma-2B-it               &            -74.1 &      -87.8 &      -73.6 &       -60.8 &        6.2 & 980        & 3.0         & 5.4        & 3.4      \\
        \bottomrule
    \end{tabular}
    }
   % }
% \textbf{Small Model:} \faCube; \textbf{Medium Model:} \faCubes; \textbf{Large Model:}  \faDiamond 
\vspace{-1em}
\end{table}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/acknowledgements.tex <==
\subsubsection*{Acknowledgments}



==> utils.tex <==
\usepackage{caption}
\usepackage{subcaption}
\usepackage[font=footnotesize, labelfont=footnotesize]{caption} 
\usepackage[font=footnotesize, labelfont=footnotesize]{subcaption} 

\newcommand{\ensuretext}[1]{#1}
\newcommand{\marker}[2]{\ensuremath{^{\textsc{#1}}_{\textsc{#2}}}}
\newcommand{\arkcomment}[3]{\ensuretext{\textcolor{#3}{[#1 #2]}}}

\definecolor{lemon}{RGB}{255,247,0}
\definecolor{maize}{RGB}{250,237,94}
\definecolor{mustard}{RGB}{255,219,89}
\definecolor{ocre}{RGB}{241,103,35}
\definecolor{Tangerine}{RGB}{253,128,8}
\definecolor{framegreen}{RGB}{153, 188, 133}
\definecolor{bggreen}{RGB}{235, 250, 228}
% \definecolor{lightgray}{RGB}{239,240,241}
\definecolor{c0}{cmyk}{1,0.3968,0,0.2588} 
\definecolor{c1}{cmyk}{0,0.6175,0.8848,0.1490} 
\definecolor{c2}{cmyk}{0.1127,0.6690,0,0.4431} 
\definecolor{c3}{cmyk}{0.3081,0,0.7209,0.3255} 
\definecolor{c4}{RGB}{164, 16, 52}
\definecolor{orange}{HTML}{E66100}
\definecolor{bluex}{HTML}{0C7BDC}
\definecolor{yellow}{HTML}{FFC20A}
\definecolor{lightpurple}{HTML}{E6E6FA}
\definecolor{lightbluee}{HTML}{e8f4f8}
\definecolor{blush}{rgb}{0.87, 0.36, 0.51}
\definecolor{c5}{HTML}{EE4E4E}
\definecolor{gggggg}{HTML}{EFEFEF}
% \definecolor{lightgray}{rgb}{0.83, 0.83, 0.83}
\definecolor{Gred}{RGB}{219, 50, 54}
\definecolor{Ggreen}{RGB}{60, 186, 84}
\definecolor{Gblue}{RGB}{72, 133, 237}
\definecolor{Gyellow}{RGB}{247, 178, 16}
\definecolor{ToCgreen}{RGB}{0, 128, 0}
\definecolor{myGold}{RGB}{231,141,20}
\definecolor{myBlue}{rgb}{0.19,0.41,.65}
\definecolor{myPurple}{RGB}{175,0,124}

\providecommand{\Comments}{1}
\ifnum\Comments>0
\usepackage[colorinlistoftodos,prependcaption,textsize=scriptsize]{todonotes}
%\setlength{\marginparwidth}{4.5cm}
\paperwidth=\dimexpr \paperwidth + 0.8cm\relax
% \oddsidemargin=\dimexpr\oddsidemargin - 2.5cm\relax
% \evensidemargin=\dimexpr\evensidemargin + 2.6cm\relax
\marginparwidth=\dimexpr\marginparwidth + 3.8cm\relax % Neurips: 1cm, ICLR: 3cm
\else
\usepackage[disable]{todonotes}
\fi
\newcommand{\mytodo}[1]{\ifnum\Comments=1{#1}\fi}
%% Inline comments:
\newcommand{\task}[1]{\mytodo{{\color{Gred}{#1}}}}
\newcommand{\chiyuaninline}[1]{\mytodo{\color{ForestGreen}[\marker CZ: #1]}}
\newcommand{\yanginline}[1]{\mytodo{\color{cyan}[\marker YH: #1]}}
\newcommand{\chulininline}[1]{\mytodo{\color{Gblue}[\marker CX: #1]}}
\newcommand{\xinyuninline}[1]{\mytodo{\color{orange}[\marker XC: #1]}}
\newcommand{\dayuinline}[1]{\mytodo{\color{ToCgreen}[\marker DY: #1]}}
\newcommand{\boinline}[1]{\mytodo{\color{Gblue}[\marker Bo: #1]}}

\newcommand{\todoinline}[1]{\todo[inline,linecolor=Gred,backgroundcolor=Gred!25,bordercolor=Gred]{#1}}

%% Margin comments
\newcommand{\badih}[1]{\todo[linecolor=Gred,backgroundcolor=Gred!25,bordercolor=Gred]{\marker BG: #1}}
\newcommand{\chiyuan}[1]{\todo[linecolor=Ggreen,backgroundcolor=Ggreen!40,bordercolor=Ggreen]{\marker CZ: #1}}
\newcommand{\yang}[1]{\todo[linecolor=cyan,backgroundcolor=cyan!10,bordercolor=cyan]{\marker YH: #1}}
\newcommand{\chulin}[1]{\ifnum\Comments<3\todo[linecolor=Gblue,backgroundcolor=Gblue!25,bordercolor=Gblue]{\marker CX: #1}\fi}
\newcommand{\bo}[1]{\ifnum\Comments<3\todo[linecolor=Gblue,backgroundcolor=Gblue!25,bordercolor=Gblue]{\marker CX: #1}\fi}
\newcommand{\dayu}[1]{\ifnum\Comments<2\todo[linecolor=Ggreen,backgroundcolor=Ggreen!25,bordercolor=Ggreen]{\marker DY: #1}\fi}
\newcommand{\ravi}[1]{\todo[linecolor=cyan,backgroundcolor=cyan!25,bordercolor=cyan]{\marker RK: #1}}
\newcommand{\xinyun}[1]{\todo[linecolor=orange,backgroundcolor=orange!25,bordercolor=orange]{\marker XC: #1}}
\newcommand{\yuchenbox}[1]{\todo[linecolor=Gyellow,backgroundcolor=Gyellow!25,bordercolor=Gyellow]{\marker YL: #1}}
\newcommand{\change}[1]{\todo[linecolor=Gred,backgroundcolor=Gred!25,bordercolor=Gred]{#1}}
\newcommand{\tableoftodos}{\ifnum\Comments=1 \listoftodos[Comments/To Do's] \fi}

% \newcommand{\chulin}[1]{\arkcomment{\marker{C}{X}}{#1}{pink}}
% \newcommand{\chiyuan}[1]{\arkcomment{\marker{C}{Z}}{#1}{ForestGreen}}
% \newcommand{\yang}[1]{\arkcomment{\marker{Y}{H}}{#1}{cyan}}
% \newcommand{\badih}[1]{\arkcomment{\marker{B}{G}}{#1}{blue}}
% \newcommand{\ravi}[1]{\arkcomment{\marker{R}{K}}{#1}{Tangerine}}
% \newcommand{\dayu}[1]{\arkcomment{\marker{D}{Y}}{#1}{blush}}


% \newcommand{\task}[1]{\textcolor{red}{TODO: {#1}}}


\usepackage{inconsolata}
\usepackage[T1]{fontenc}
\usepackage[scaled=0.95]{biolinum}




\usepackage{tcolorbox}
\definecolor{chart}{HTML}{1f77b4}
\newcommand{\chartcolor}[1]{\textcolor{chart}{#1}}
\newtcolorbox{example}[1][]{
  colback=chart!5!white,
  colframe=chart,
  floatplacement=floating,
  title=\centering \textsf{\small #1}
}


\newtcbox{\hlprimarytab}{on line, box align=base, colback=BlueGreen!20,colframe=blue,size=fbox,arc=3pt, before upper=\strut, top=-2.5pt, bottom=-4.5pt, left=-2pt, right=-2pt, boxrule=0pt}
\newtcbox{\hlsecondarytab}{on line, box align=base, colback=WildStrawberry!10,colframe=orange,size=fbox,arc=3pt, before upper=\strut, top=-2.5pt, bottom=-4.5pt, left=-2pt, right=-2pt, boxrule=0pt}
\newtcbox{\hlwhite}{on line, box align=base, colback=WildStrawberry!8,colframe=white,size=fbox,arc=2pt, before upper=\strut, top=-3pt, bottom=-4.5pt, left=-2pt, right=-2pt, boxrule=0pt}
\newtcbox{\hlyellow}{on line, box align=base, colback=BlueGreen!10,colframe=white,size=fbox,arc=2pt, before upper=\strut, top=-3pt, bottom=-4.5pt, left=-2pt, right=-2pt, boxrule=0pt}

\newcommand{\uashifted}{{\tiny$\uparrow$}}
\newcommand{\dashifted}{{\tiny$\downarrow$}}
\newcommand{\ua}[1]{{\scriptsize\hlsecondarytab{\uashifted{#1}}}}
\newcommand{\da}[1]{{\scriptsize\hlprimarytab{\dashifted{#1}}}}
\newcommand{\dae}[1]{{\scriptsize{\dashifted{#1}}}}
\newcommand{\dar}[1]{{\scriptsize\hlsecondarytab{\dashifted{#1}}}}
\newcommand{\uar}[1]{{\scriptsize\hlprimarytab{\uashifted{#1}}}}

\newcommand{\orange}[1]{{\hlsecondarytab{#1}}}
\newcommand{\blue}[1]{{\hlprimarytab{#1}}}
\newcommand{\white}[1]{{\hlwhite{\textcolor{black}{\scriptsize\texttt{#1}}}}}
\newcommand{\yellow}[1]{{\hlyellow{\textcolor{black}{\scriptsize\textsf{#1}}}}}


\newcommand*{\affmark}[1][*]{\textsuperscript{\textnormal{#1}}}

\usepackage{titletoc}
\usepackage{fontawesome}



\usepackage{tcolorbox}



\newtcolorbox{promptbox}[1][]{%
  colback=blue!10,
  colframe=blue!30!black,
  fonttitle=\bfseries,
  title=#1, % Use the optional argument as the title
  sharp corners,
  % breakable,
    fontlower=\scriptsize, % Reduce font size
 % boxrule=0.5pt, % Reduce border thickness
  boxsep=1mm, % Reduce internal margin
 %  left=0mm, % Reduce left margin
 %  right=0mm, % Reduce right margin
 %  top=0mm, % Reduce top margin
 %  bottom=0mm % Reduce bottom margin
}



